Statistical Model Checking for Hyperproperties

Hyperproperties have shown to be a powerful tool for expressing and reasoning about information-flow security policies. In this paper, we investigate the problem of statistical model checking (SMC) for hyperproperties. Unlike exhaustive model checking, SMC works based on drawing samples from the system at hand and evaluate the specification with statistical confidence. The main benefit of applying SMC over exhaustive techniques is its efficiency and scalability. To reason about probabilistic hyperproperties, we first propose the temporal logic HyperPCLT* that extends PCTL* and HyperPCTL. We show that HyperPCLT* can express important probabilistic information-flow security policies that cannot be expressed with HyperPCTL. Then, we introduce SMC algorithms for verifying HyperPCLT* formulas on discrete-time Markov chains, based on sequential probability ratio tests (SPRT) with a new notion of multi-dimensional indifference region. Our SMC algorithms can handle both non-nested and nested probability operators for any desired significance level. To show the effectiveness of our technique, we evaluate our SMC algorithms on four case studies focused on information security: timing side-channel vulnerability in encryption, probabilistic anonymity in dining cryptographers, probabilistic noninterference of parallel programs, and the performance of a randomized cache replacement policy that acts as a countermeasure against cache flush attacks.

==> backup.tex <==
% \subsection{Strict}


%

%
% This is because SPRT, although very efficient, can only distinguish between two distinctive points in the two test regions; and as shown in \cref{fig:ht}, 
% the assumption ensures that there is a ``gap'' between the two test regions, so they have such distinctive hypothesis points in the worst case.
% %
% \begin{assumption} \label{ass:indifference}
% 	For checking~\eqref{eq:hypothesis test}, either $(\m, X, V) \models (p_{\varphi_1}, \ldots, p_{\varphi_n}) \in D_0$ or $(\allowbreak \m, X, V) \models (p_{\varphi_1}, \ldots, p_{\varphi_n}) \in D_1$ holds for some $D_0 \subseteq D \subseteq D_1$ with $d_H(D_0, D) > 0$ and $d_H(D_1, D) > 0$.
% \end{assumption}
% %
% Due to \cref{ass:indifference}, verifying $(\P^{\pvs_1} \varphi_1, \ldots, \P^{\pvs_n} \varphi_n) \allowbreak \in D$ is equivalent to verifying $(\P^{\pvs_1} \varphi_1, \ldots, \P^{\pvs_n} \varphi_n) \in D'$, if $\overline{D} = \overline{D'}$, thus they will not be distinguished in the rest of the paper.




% To calculate the statistical significance of the above assertion, we consider the log-likelihood for an arbitrary hypothesis $\underline{p} = (p_1, \ldots, p_n)$ for the given samples
% \begin{equation} \label{eq:Lambda}
% 	\Lambda(\underline{p}) =  \ln \big(p_i^{T_i} (1 - p_i)^{N_i - T_i} \big) = T_i \ln p_i + (N_i - T_i) \ln (1 - p_i)  
% \end{equation}
% whose gradient is 
% \begin{equation} \label{eq:Lambda_gradient}
% 	\underline{\lambda} = \nabla \Lambda(\underline{p}) = \big(\frac{N_1 (q_1 - p_1)}{p_1 (1 - p_1)}, \ldots, \frac{N_1 (q_1 - p_1)}{p_1 (1 - p_1)} \big)  
% \end{equation}
% %
% For simplicity, let $\underline{q} \in D_0$ (the treatment for $\underline{q} \in D_1$ is similar),
% then the maximal-likelihood hypothesis point under the hypothesis $H_1$ is
% \begin{equation} \label{eq:q1}
% 	\underline{q_1} = \argmax_{\underline{p} \in H_1} \Lambda(\underline{p})  
% \end{equation}
% which can be solved by finding $\underline{q_1}$ whose tangent hyperplane $l_1$ of $D_1$ is orthogonal $\underline{\lambda}$.
% %
% This hypothesis point is compared with its ``closest'' hypothesis point in $D_0$, whose tangent hyperplane $l_0$ of $D_0$ is orthogonal to $\underline{\lambda}$ and separates $\underline{q_1}$ and $D_0$. 



% \begin{equation} \label{eq:Lambda}
% 	\begin{split}
% 		& \Lambda = \Lambda_1 / \Lambda_0, 
% 		\quad \Lambda_1 = \max_{(p_{\varphi_1}, \ldots, p_{\varphi_n}) \in D^{\mathrm{c}}_1} \prod_{i \in [n]} p_{\varphi_i}^{T_i} (1 - p_{\varphi_i})^{N_i - T_i}
% 		\\ & 
% 		\quad \Lambda_0 = \max_{(p_{\varphi_1}, \ldots, p_{\varphi_n}) \in D_0} \prod_{i \in [n]} p_{\varphi_i}^{T_i} (1 - p_{\varphi_i})^{N_i - T_i},
% 	\end{split}
% 	\end{equation}




\subsection{Difficulty in finding conservative SPRT-based SMC algorithms}


Sequential likelihood ratio test (SPRT) is a commonly used conservative statistical test to distinguish between two \emph{simple} hypothesis, based on the condition that one of the two simple hypothesis always holds.
%
Specifically, assume that in the hypothesis testing problem~\eqref{eq:hypothesis test}, $\underline{p_0} \in D$ and $\underline{p_1} \in D^{\mathrm{c}}$ are the only pair of candidates, namely, we somehow know that $\underline{p_\varphi}$ has to be either $\underline{p_0}$ or $\underline{p_1}$, then the two simple hypothesis $\underline{p_\varphi} = \underline{p_0}$ and $\underline{p_\varphi} = \underline{p_1}$ can be tested with (conservative) guarantees on the FP and FN ratios by
\begin{equation} \label{eq:sprt}
	\begin{cases}
		\text{assert } H_0, & \text{ if } \lambda(\underline{p_1}) - \lambda(\underline{p_0}) < \ln \frac{\FP}{1 - \FN} \textrm{ for the first time} \\
		\text{assert } H_1, & \text{ if } \lambda(\underline{p_1}) - \lambda(\underline{p_0}) > \ln \frac{1 - \FP}{\FN} \textrm{ for the first time} \\
		\text{draw more samples}, & \text{ otherwise,}
	\end{cases}
\end{equation}
where 
\begin{equation}
	\lambda(\underline{p}) = \ln \Big( \prod_{i \in [n]} p_i^{T_i} (1 - p_i)^{N_i - T_i} \Big), \quad \underline{p} = (p_1, \ldots, p_n) 
\end{equation}
is the log-likelihood of the drawn samples $\{(N_i, T_i)\}_{i \in [n]}$ using the the simple hypothesis $\underline{p_\varphi} = \underline{p}$.



Without such assumptions, solving the hypothesis testing problem~\eqref{eq:hypothesis test} is notoriously difficult with conservative guarantees on the FP and TN ratios~\cite{lai_SequentialAnalysisClassical_2001}.
%
This is because in~\eqref{eq:hypothesis test}, both the hypothesis $H_0$ and $H_1$ are composite and there are infinitely many such pairs of candidates, but SPRT can only test between one of them at a time.
%
% Therefore, to conservatively test between $H_0$ and $H_1$, the SPRT test should run over all possible $\underline{p_0} \in D$ and $\underline{p_1} \in D$, which is computationally impossible.



It was believed that under certain assumption on the difference region, we can identify the two most ``indistinguishable'' \emph{simple} hypothesis in $H_0$ and $H_1$.
%
Specifically, in the $1$-D case that $\underline{p_\varphi} = p_\varphi \in [0, 1]$, assume there exists an indifference region $(p_l, p_u) \subseteq [0,1]$ such that $p_\varphi \notin (p_l, p_u)$, 
%
It is believe that if we run the SPRT of~\eqref{eq:sprt} between $p_\varphi = p_l$ and $p_\varphi = p_u$,
then upon termination, the LL ratio $\Lambda$ for any pair of simple hypothesis from $H_0$ and $H_1$ is bounded by $\Lambda \geq \lambda(p_u) - \lambda(p_l)$ if $p_\varphi \geq p_u$; and $\Lambda \leq \lambda(p_l) - \lambda(p_u)$ if $p_\varphi \geq p_l$.
%
Therefore, the SPRT distinguishing $p_\varphi \in p_l$ and $p_\varphi \in p_u$ is guaranteed to distinguish any pair of hypothesis from $H_0$ and $H_1$ with no less accuracy.
%
We provide the following counter-example to show this belief, although true in most cases, can be wrong in extreme cases.



\paragraph*{Counter-example}.
Let $p_l = 0.1$, $p_u = 0.3$, $p_\varphi = 0.5$ and $\FP = \FN = 0.5 - \varepsilon$.
%
For sufficiently small $\varepsilon$, the SPRT~\eqref{eq:sprt} always stop for one sample.
%
Therefore, as $p_\varphi = 0.5$, the sample is $0$ or $1$ with equal probability, thus the actual FP an FN ratios are both $0.5$, which are greater than desired.












As a well-known result, the probability distribution of $2 \abs{\Lambda_M}$ converges that of the $\chi^2(1)$ distribution. Therefore, we design the following sequential

As $\Lambda$ or equivalently $\ln(\Lambda)$ increases, $H_1$ is more likely to hold; otherwise, $H_0$ is more likely to hold. 
%
The sequential SMC algorithm is designed by assigning an upper $A$ and an lower bound $B$ on $\Lambda$, and monitor the value of $\Lambda$ as samples gather.
%
If $\ln(\Lambda)$ grows above $A$, then the sampling stops and $H_1$ is returned; if $\ln(\Lambda)$ drops below $B$, then the sampling stops and $H_0$ is returned;
otherwise, the sampling continues.  
%
Similar to SPRT, the SMC algorithm has false positive (FP) and true negative (TN) ratios $\alpha$ and $\beta$ if $A =\ln((1 - \beta)/\alpha)$ and $B = \ln(\beta/(1 - \alpha))$.
%
This is summarized by~\cref{alg:non-nested} and~\cref{thm:sequential}.

==> prelim.tex <==
%TEX root=main.tex

\section{Preliminaries}
\label{sec:prelim}

% \todo{BB: consider merging.}


%
% Given a map $V: A \rightarrow B$ and $A' \subset A$, let $V(A') = \{V(a) \mid a \in A'\}$.
%
% We denote by $d_H(\cdot, \cdot)$ the {\em Hausdorff} distance on the Euclidean space.
%
% The domain and range of a mapping are denoted by $\dom(\cdot)$ and $\ran(\cdot)$, respectively.  





% \subsection{Sequential Probability Ratio Test (SPRT)}
% \label{sub:sprt}





% \paragraph{Clopper-Pearson Significance Level}

% Let $T \sim \bin(N, p)$.
% Intuitively, if $T / N \in [a,b]$ for some $a < b \in [0,1]$,
% then it is likely that the assertion $p \in [a, b]$ holds.
% The significance level for making such an assertion can be computed using the
% Clopper-Pearson (CP) method as:
% \begin{equation} \label{eq:cp}
% \begin{split}
% 	& \alpha_{\text{CP}} (a, b \, \vert \, T, N) = 1 -
% 	\begin{cases}
% 	(1-a)^{N} - (1-b)^{N}
% 	& \text{ if } T = 0 \\
% 	b^{N} - a^{N}
% 	& \text{ if } T = N \\
% 	F_\text{Beta} ( b \, \vert \, T+1, N\hspace{-2pt} -\hspace{-2pt} T ) -
% F_\text{Beta} ( a \, \vert \, T, N\hspace{-2pt} -\hspace{-2pt} T +\hspace{-2pt}
% 1 )
% 	& \text{ otherwise.}
% \end{cases}
% \end{split}
% \end{equation}
% Here, $F_\text{Beta}(\cdot \, \vert \, \alpha, \beta)$ denotes the cumulative probability of the beta distribution with the shape parameters $(\alpha, \beta)$.
